Verification and Parameter Synthesis for Real-Time Programs using Refinement of Trace Abstraction

We address the safety verification and synthesis problems for real-time systems. We introduce real-time programs that are made of instructions that can perform assignments to discrete and real-valued variables. They are general enough to capture interesting classes of timed systems such as timed automata, stopwatch automata, time(d) Petri nets and hybrid automata. We propose a semi-algorithm using refinement of trace abstractions to solve both the reachability verification problem and the parameter synthesis problem for real-time programs. All of the algorithms proposed have been implemented and we have conducted a series of experiments, comparing the performance of our new approach to state-of-the-art tools in classical reachability, robustness analysis and parameter synthesis for timed systems. We show that our new method provides solutions to problems which are unsolvable by the current state-of-the-art tools.

==> results/reachability.tex <==

\begin{tabular}{|l|r|r|r|r|}
\hline
Test&\multicolumn{2}{c|}{Time}\\\hline\hline
&{\uppaal}&{\tar}\\\hline
\hline
\texttt{csma\_05}&0.03&88.26\\\hline
\texttt{csma\_06}&0.07&350.36\\\hline
\texttt{csma\_07}&0.26&1128.26\\\hline

\texttt{fischer\_04}&0.02&15.71\\\hline
\texttt{fischer\_05}&0.02&69.20\\\hline
\texttt{fischer\_06}&0.06&641.47\\\hline

\texttt{hddi\_12}&17.58&0.03\\\hline
\texttt{hddi\_13}&71.42&0.20\\\hline
\texttt{hddi\_15}&720.38&0.14\\\hline

\end{tabular}

==> robustness.tex <==
%!TEX root = ./main.tex

In this section we show how to use the trace abstraction refinement algorithm presented in Section~\ref{sec:tar} to check whether a real-time program is \emph{robust}. Notice that we can check robustness of real-time program so this is not limited to timed automata. \emph{Shrinking} and \emph{sampling} semantics can also be handled with our method. We focus here on robustness.
%
For an overview of robustness for timed automata see~\cite{phd-sankur}.

\paragraph{\bfseries Enlargement.}
Given a positive real number $\varepsilon$, an \emph{enlargement} $\varphi_\varepsilon$ of a constraint $\varphi \in \bexpr(V)$ is a \emph{widening} of $\varphi$.  We only require  $\varphi_\varepsilon$ to be \emph{weaker} than $\varphi$, \ie $\forall \nu \in [V \rightarrow \setR], \nu \models \varphi \implies \nu \models \varphi_\varepsilon$.

As an example, triangular constraints (Equation~\eqref{eq-grammar-ta}) are enlarged as per \tabref{tab-enlarge} ($\bowtie \in \{<,\leq\}, k \in \setQ_{\geq 0}$.)
\begin{table}[thbp]\centering
\begin{tabular}{||p{2cm}|p{3.3cm}||}\hline\hline
	$\varphi$ & $\varphi_\varepsilon$ \\ \hline\hline
	$x - y \bowtie k$  & $x - y \bowtie k + \varepsilon$ \\
	$k \bowtie x - y$  & $k - \varepsilon \bowtie x - y$ \\
	$x - y = k$  & $k - \varepsilon \leq  x - y \leq k + \varepsilon$ \\
	$b \wedge b'$ & $b_\varepsilon \wedge b'_\varepsilon$ \\
	$\true$ & $\true$ \\
	$\false$ & $\false$ \\ \hline\hline
\end{tabular}
\caption{Enlargement of contraints for the grammar of Equation~\eqref{eq-grammar-ta}}
\label{tab-enlarge}
\end{table}

%\paragraph{\bfseries Robust Emptiness.}
%Given a real-time program $(A,\calT)$, a constant value $\varepsilon > 0$ we let $(A,\calT_\varepsilon)$ be the real-time program with all the constrainsts in $\calT$ enlarged by $\varepsilon$.
%%
%The \emph{robust language emptiness problem}~\cite{DBLP:journals/fmsd/WulfDMR08} asks the following:
%\begin{quote}
%	Given a real-time program $(A,\calT)$, is there $\varepsilon\!>\!0$ such that $\tlang(A,\calT_\varepsilon) = \varnothing$?
%\end{quote}
%Because we enlarge the guards, and by definition of word feasibility, if $\varepsilon' \leq \varepsilon$ then $\tlang(A,\calT_{\varepsilon'}) \subseteq \tlang(A,\calT_\varepsilon)$.
%This implies the following:
%\begin{lemma}[see~\cite{}]
%	The set of values of $\varepsilon$ such that $\tlang(A,\calT_\varepsilon) \neq \varnothing$ and $\varepsilon > 0$ is either 1) empty or 2) \emph{upwards closed} \ie
%a set of the form $\varepsilon \bowtie r$ with $r \in \setR_{\geq 0}$ and $\bowtie \in \{>, \geq\}$.
%\end{lemma}
%
%%
%\paragraph{\bfseries Semi-Algorithm for the Robust Emptiness Problem.}
%Let $\pi$ be a fresh letter not in $\Sigma$.
%Given an automaton $A=(Q,q_0,\Sigma, \Delta,F)$, we define automaton $A_\pi=(Q \cup \{q_{-1}\},q_{-1},\Sigma\cup \{\pi\}, \Delta \cup \{(q_{-1},\pi,q_0)\}, F)$ \ie from its initial location $q_{-1}$, there is only one outgoing transition labeled $\pi$; the target location is the initial location of $A$.
%
%This $\pi$ label (instruction) is meant to impose the initial contraint on the possible values of $\varepsilon$ which we define  as $r > 0$ where $r \not\in V$ is the robustness variable (with derivative $0$ for each label).
%
%The semi-algorithm \figref{fig-rob-emptiness} performs an iterative search by removing the values of $\varepsilon$ for which $\tlang(A,\calT_\varepsilon) \neq \varnothing$.
%This iterative search means that we strenghten the initial constraint on $\varepsilon$ at each new iteration.
%
%We define the \emph{parametric} mapping $\calT(g): \alphabet \cup \pi \rightarrow \bexpr(\rvars \cup \{r\}) \times \calU(\rvars \cup \{r\}) \times \calR(\rvars \cup \{r\})$, for
%$g$ be a constraint on $r$, as follows:
%\begin{itemize}
%	\item for $\lbl \in \Sigma$, if $\calT(\lbl) = (\varphi,\mu,\gamma)$, then $\calT(g)(\lbl) = (\varphi,\mu,\gamma')$ with $\gamma'(v) = \gamma(v)$ for $v \in V$ and $\gamma'(r)=0$; (the rate of $r$ is always $0$.)
%	\item for $\alpha=\pi$, $\calT(g)(\alpha) = (g,Id,\gamma)$ with $\gamma(v) = 0$ for $v \in V \cup \{r\}$ (the instruction $\pi$ constrains $r$ and does not update any variable.)
%	\end{itemize}
%
%\begin{figure}[thbp]
%\centering
%\begin{tikzpicture}[scale=1,node distance=1.4cm and 1.5cm, very thick, bend angle=20,bend angle=10]
%\fontsize{10}{11}\selectfont
%\tikzset{green/.style={rectangle, rounded corners,thick,draw=black},
%    red/.style={rectangle, rounded corners,thick,draw=black},
%    adam/.style={rectangle, rounded corners,thick,draw=black},
%    module/.style={rectangle, rounded corners,thick,draw=black}}
% \node[module](0,0) (init) {\textbf{1:} $\tlang(A_\pi,\calT(g)) = \varnothing$?};
% \node[module,right of=init, xshift=6.5cm] (step2) {
% 	\textbf{2:} $g \wedge \neg I(w) = \false$?};
%  \node[below of=init,xshift=-0cm] (nobug) {$g$};
%  \node[below of=step2, yshift=-.0cm] (bug) {$g := \false$};
%  \node[above of=init,xshift=-1.9cm] (start) {$g := r > 0$};
%\node[right of=start,yshift=0cm,xshift=4cm,module] (step3) {\textbf{3:} $g := g \wedge \neg I(w)$};
%
%\path[->] (init) edge[draw=black,swap] node {\textbf{Yes}} (nobug)
%                edge[swap] node[yshift=.46cm] {
%				\begin{tabular}{c}
%					\textbf{No} \\ Let $w \in \lang(A_\pi)$ such that \\ $\tau(w) \cap \lang(A_\pi,\calT(g)) \neq \varnothing$
%				\end{tabular}} (step2);
%
% \draw[->] (step2) |- node[xshift=0.4cm,yshift=-.5cm] {\textbf{No}}  (step3.east);
% \draw[->] (step2) edge node[xshift=0cm] {\textbf{Yes}}  (bug);
% \draw[->] (step3.west) -| ($(init.north) + (0cm,0)$);
% \draw[->] (start) -|  ($(init.north) + (-.6cm,0)$);
%\end{tikzpicture}
%% \vspace{-2.8em}
%\caption{Semi-algorithm $CheckRobustness$.}
%\label{fig-rob-emptiness}
%\end{figure}
%%
%\noindent The algorithm \figref{fig-rob-emptiness} works as follows:
%\begin{enumerate}
%	\item initially $g = r > 0$;
%	\item if $\tlang(A_\pi,\calT(g))$ is empty then every value of $r$ that satisfies $g$
%	 is such that $\tlang(A,\calT_r)=\varnothing$;
%	\item otherwise, there is a witness word $w \in \lang(A_\pi)$ such that $\tau(w) \cap \tlang(A_\pi,\calT(g)) \neq \varnothing$.
%	The enconding of $w$ is $\enc(w)=g \wedge P_0 \wedge P_1 \wedge \cdots \wedge P_n$ and has variables in $ \{r\} \bigcup \cup_{0 \leq i \leq n}\vars(P_i)$ (as $r$ is never updated in $A_\pi$ we do not need $r_{-1}, r_0, \cdots r_n$).
%	We define the existentially quantified predicated $I(w) = \exists \vars(w) \setminus \{r\}$.
%	This must define an upwards closed set (fact~\ref{fact-up-closed}). For each value $\varepsilon$ in this set, $w$ is witness for $\tlang(A,\calT_\varepsilon) \neq \varnothing$.
%	\item if $g \wedge I(w)$ is empty, there is no $\varepsilon>0$ such that $\tlang(A,\calT_\varepsilon) = \varnothing$. Otherwise, we continue for $\varepsilon$, but we know it must be outside $I(w)$.
%	$g$ is updated to $g \wedge \neg I(w)$.
%	%
%	%  or not (use the trace abstraction refinement from previous section); the contraint on $\varepsilon$ is given by $g$ and it $\varepsilon >0$ initially.
%	% \item if it is empty, then $g$ is the largest constraint for which  $\tlang(A_\pi,\calT_\varepsilon)$  is empty and we output $g$;
%	% if it is not empty, we have a timed word $w$ that is accepted by $(A,\calT_\varepsilon)$. We can compute a constraint on $\varepsilon$, $I_\varepsilon(w)$, for which the timed word is feasible. This constraint must define an upwards closed set (\eg $\varepsilon>2$ or $\varepsilon\geq2$). We know that for all the enlargements $\varepsilon'$ in $I_\varepsilon(w)$,
%	% $\tlang(A_\pi,\calT_{\varepsilon'}) \neq \varnothing$. So $I_\varepsilon(w)$ is not a good set of values and is discarded in the next round (step 3). We are now looking for a value of $\varepsilon$ that is not in the values we have discarded before.
%	% \item if the algorithm terminates, it gives the largest set of $\varepsilon$ (encoded in $g$) such that $\tlang(A_\pi,\calT_\varepsilon)$ is empty (works for stopwatch automata as well).
%	% \item notice that if $g = \false$ (there is no enlargement) we can avoid checking step 1 again.
%	% If we do check step 1 we will find that $\tlang(A_\pi,\calT_\varepsilon)$ is empty and stop.
%\end{enumerate}
%Algorithm $CheckRobustness$ when it terminates, computes the maximal set of values $\varepsilon$ for which  $\tlang(A,\calT_\varepsilon) = \varnothing$. This is a consequence of Theorem~\ref{thm-max-rob}:
%\begin{theorem}\label{thm-max-rob}
%If  algorithm $CheckRobustness$ terminates,
%\begin{enumerate}
%	\item $\semof{g}$ is either empty or a set of positive values of the form $0 < r \bowtie k$ with $\bowtie \in \{<, \leq\}$ and $k \in \setR_{\geq 0} \cup +\infty$;
%	\item $\tlang(A,\calT_r) = \varnothing$ if and only if $r \in \semof{g}$.
%\end{enumerate}
%\end{theorem}
%\begin{proof}
%	\textbf{1.} is an invariant of algorithm $CheckRobustness$: initially $g$ is $0 < r < +\infty$.
%	Each $I(w)$ is an upward closed set. When $I(w)$ is removed from $g$ is generates a set of the desired form.
%
%	\textbf{2.} If algorithm $CheckRobustness$ terminates in $0$ iteration, then $g = r > 0$ and this is the maximal set of values for which $\tlang(A,\calT_r) = \varnothing$.
%
%	If algorithm $CheckRobustness$ terminates in $k \geq 1$ iterations, we have discovered a finite number of words $w_1, \cdots, w_k$ and the final value of $g$ is $g_f = (r > 0) \wedge \neg I(w_1) \wedge \neg I(w_2) \wedge \cdots \wedge \neg I(w_k)$. $g_f$ is equivalent to
%	$(r > 0) \wedge \neg (I(w_1) \vee  I(w_2) \vee \cdots \vee  I(w_k))$.
%	Assume $\tlang(A,\calT_r) = \varnothing$ for $0 < r \not\in \semof{g_f}$. Then $r$ must be in
%	$I(w_1) \vee  I(w_2) \vee \cdots \vee  I(w_k)$. But each $w_i$ is such that  $x \in I(w_k)$ implies $\tlang(A,\calT_x) \neq \varnothing$, which is a contradiction.
%	\qed
%\end{proof}
%
 \paragraph{\bfseries Maximal Robustness Example.}
We illustrate the computation of the maximal enlargement value on automaton $A_1$.
The enlarged guards are $1 - r \leq x \leq 1 + r$ and $x - y \geq 1 -r \wedge z < 1 + r$.
%
Step \textbf{1:} of algorithm $CheckRobustness$ produces the witness word $w_1= \pi.i.t_0.t_2$.
The encoding of the feasibility of $w_1$ (with $r$ the enlargement) as a SMT-problem is:
\begin{align}
	 r &> 0  \label{eqr-0} \tag{$Z_{-1}$} \\
     x_0 &=  y_0 = z_0 = \delta_0 \wedge \delta_0 \geq 0 & \label{eqr-1} \tag{$Z_0$} \\
     x_1 &=  x_0 + \delta_1 \wedge y_1 = y_0 \wedge z_1 = \delta_1 \wedge \delta_1 \geq 0 &  \label{eqr-2} \tag{$Z_1$}  \\
     x_1  &-  y_1 \geq 1 - r \wedge z_1 < 1 + r \wedge x_2 = x_1 + \delta_2 \wedge y_2 = y_1 \wedge  z_2 = z_1 + \delta_2 \wedge \delta_2 \geq 0 & \label{eqr-3} \tag{$Z_2$}
\end{align}
This formula is satisfiable (this can be checked with Z3). The theory of Linear Real Arithmetic (LRA), admits quantifier elimination~\cite{}, and we can effectively remove the existential quantifier in $I(w_1)$ which gives: $I(w_1) = r > 0$. The updated value of $g$ is $g := (r > 0) \wedge \neg (r > 0)$ which is equivalent to $\false$. Hence no parameters exist\footnote{We can run our algorithm we the initial constraint $r \geq 0$ instead of $r > 0$. In this case $CheckRobustness$ compute the final value of $g$ is $r = 0$. Theorem~\ref{thm-max-rob} can be refined to integrate $r =0$.} to preserve emptiness.

Now assume we modify the ``Guard'' entry  for $t_2$ in Table in \figref{fig-ex1} as follows: $x - y \geq 2 \wedge z < 1$. Let $t_2'$ denote the new entry and $A_1'$ the new program.
Running $CheckRobustness$ on $A_1'$ produces $w_1= \pi.i.t_0.t_2'$.
The set $I(w_1)$ is $r > 1/2$. The test $\tlang(A_\pi,\calT(r > 1/2)) = \varnothing$ terminates
and is positive. Hence the maximal set of values for which $A_1'$ is robust is $0 < r \leq 1/2$.
The interpolants that are discovered during this test are $x -y \geq 2 \wedge z < 1 \wedge 0 < r < 1/2$.

Notice that the semi-algorithms and tools~\cite{sankur-tacas-15,verifix} cannot compute the results
on $A_1, A_1'$ because there are  stopwatch automata and these tools are limited to timed automata. Note also that \phaver will not converge if we add a new stopwatch $r$ and is unable to produce the results.

